SPIRE Map-Making Test Report

The photometer section of SPIRE is one of the key instruments on board of Herschel. Its legacy depends very much on how well the scanmap observations that it carried out during the Herschel mission can be converted to high quality maps. In order to have a comprehensive assessment on the current status of SPIRE map-making, as well as to provide guidance for future development of the SPIRE scan-map data reduction pipeline, we carried out a test campaign on SPIRE map-making. In this report, we present results of the tests in this campaign.

==> chapter3_testcases.tex <==
\chapter{Test Cases}
, sampling rate = 10 Hz).
Test cases were designed under that following guide lines:
\begin{itemize}
\item They shall cover the following parameter space of SPIRE scanmap 
observations: 
(1) observation mode (nominal/parallel, scan speed, sampling rate); 
(2) source brightness; 
(3) map size; 
(4) depth; 
(5) complexity of the extended emission.
\item They shall include examples of: 
(i) observations suffering from the "cooler burp" effects; 
(ii) sky regions with strong large-scale gradient. 
\end{itemize}

In total 13 test cases were generated. As shown in Table\ref{tbl:testcases},
they include both real observations
(5 cases) and simulated observations (8 cases) in 4 observational
modes. In the nominal mode (scan speed = 30$”$/sec, sampling rate = 16
Hz), we have 5 test cases (2 real, 3 simulated). In the fast-scan mode
(scan speed = 60$”$/sec, sampling rate = 16 Hz), there are 3 test
cases (1 real, 2 simulated). In the parallel mode (sampling rate = 10 Hz), 
we have 4 test cases (1 real, 3
simulated) in slow scan (scan speed = 20$”$/sec) 
and 1 real case in fast-scan (scan speed = 60$”$/sec).

%\begin{savenotes}
\begin{table}[ht]
\begin{minipage}{\textwidth}  % this is to have the footnote!!!
\renewcommand\footnoterule{}
\caption[Caption for LOF]{Summary of Test Cases\label{tbl:testcases}
}
\centering
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\bf{Case} & &\bf{Name} & \be{Mode} & scan speed & sampling &\bf{Size} \\ 
\hline
          & &          &           & arcsec/sec & Hz       &(deg$\times$deg) \\
\hline
1 & simulation & Nominal~Sources     & Nominal & 30 & 16 & 0.7$\times$0.7 \\
\hline
2 & simulation & Nominal~Cirrus      & Nominal & 30 & 16 & 0.7$\times$0.7 \\ 
\hline
3 & real~obs   & Nominal~Dark        & Nominal & 30 & 16 & 0.7$\times$0.7 \\
\hline
4 & simulation & Nominal~M51         & Nominal & 30 & 16 & 0.7$\times$0.7 \\
\hline
5 & simulation & Fast-scan~Sources   & Fast~Scan & 60 & 16 & 3.5$\times$3.5 \\
\hline
6 & simulation & Fast-scan~MK-Center & Fast~Scan & 60 & 16 & 3.5$\times$3.5 \\
\hline
7 & real~obs   & Fast-scan~Dark      & Fast~Scan & 60 & 16 & 3.5$\times$3.5 \\
\hline
8 & simulation & Parallel~Sources    & Parallel & 20 & 10 & 1.3$\times$1.3 \\ 
\hline
9 & simulation & Parallel~MK-Center  & Parallel & 20 & 10 & 1.3$\times$1.3 \\ 
\hline
10 & simulation& Parallel~Cirrus     & Parallel & 20 & 10 & 1.3$\times$1.3 \\ 
\hline
11 & real~obs  & Parallel~Dark       & Parallel & 20 & 10 & 1.3$\times$1.3 \\ 
\hline
12 & real~obs  & Nominal~NGC~628     & Nominal & 30 & 16 & 0.4$\times$0.4 \\
\hline
13 & real~obs  & Para-fast~Hi-Gal-L30& Parallel & 60 & 10 & 1.9$\times$1.9 \\
\hline
\end{tabular}
\end{minipage}
\end{table}
%\end{savenotes}


%\begin{savenotes}
\begin{table}[ht]
\begin{minipage}{\textwidth}  % this is to have the footnote!!!
\renewcommand\footnoterule{}
\caption[Caption for LOF]{Summary of Test Cases as Processed by Different Map-Makers}
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\bf{Case} & \bf{Description} & \bf{Size} & \multicolumn{7}{|c|}{{\bf Map-Maker}\protect\footnote{Abbreviations for map-makers: N -- Naive, D -- Destriper, Sc -- Scanamorphos, SA -- SANEPIC, U -- Unimap, H -- HiRes, SU -- SUPREME.}\label{tbl:testcases}
} \\ 
\hline
          &      &(deg$\times$deg) & N & D & Sc & SA & U & H & SU \\ 
\hline
1 & Nominal Sources & 0.7$\times$0.7 & $\surd$& $\surd$& $\surd$& $\surd$& $\surd$ & & \\
\hline
2 & Nominal Cirrus & 0.7$\times$0.7 & $\surd$& $\surd$& $\surd$& $\surd$&  & & \\
\hline
3 & Nominal Dark & 0.7$\times$0.7 & $\surd$& $\surd$& $\surd$& $\surd$& & & \\
\hline
4 & Nominal M51 & 0.7$\times$0.7 & $\surd$& $\surd$& $\surd$& $\surd$& & & \\
\hline
5 & Fast-scan Sources & 3.5$\times$3.5 & $\surd$& $\surd$& $\surd$& $\surd$& $\surd$ & & \\
\hline
6 & Fast-scan MK Center & 3.5$\times$3.5 & $\surd$& $\surd$& $\surd$& $\surd$& $\surd$ & & \\
\hline
7 & Fast-scan Dark & 3.5$\times$3.5 & $\surd$& $\surd$& $\surd$& $\surd$&  & & \\
\hline
8 & Parallel Sources & 1.3$\times$1.3 & $\surd$& $\surd$& $\surd$& $\surd$&  & & \\
\hline
9 & Parallel Mk Center & 1.3$\times$1.3 & $\surd$& $\surd$& $\surd$& $\surd$&  & & \\
\hline
10 & Parallel Cirrus & 1.3$\times$1.3 & $\surd$& $\surd$& $\surd$& $\surd$& $\surd$& $\surd$& $\surd$ \\
\hline
11 & Parallel Dark & 1.3$\times$1.3 & $\surd$& $\surd$& $\surd$& $\surd$&  & & \\
\hline
12 & Nominal NGC~628 & 0.4$\times$0.4 & $\surd$& $\surd$& $\surd$& & $\surd$& $\surd$& \\
\hline
13 & Para-fast Hi-Gal L30 & 1.9$\times$1.9 & $\surd$& $\surd$& $\surd$& & $\surd$& $\surd$& \\
\hline
\end{tabular}
\end{minipage}
\end{table}
%\end{savenotes}



The input data for the map-making tests, in all these test cases, are
time-ordered data, or TOD. The map-making process turns the TOD
into maps. These TOD have the format of the SPIRE Level-1 Photometer
Scan Product (PSP). They were corrected for the following instrumental
effects using the standard SPIRE scanmap data reduction pipeline:
\begin{itemize}
\item	glitches;
\item	electrical low-pass filter;
\item	non-linearity;
\item	bolometer time response.
\end{itemize}

For each test case, two sets of input data were generated: 
\begin{description}
\item{Set-1:} The
TOD were also corrected for the detector array temperature drift using
the standard pipeline; and the “turn-around” data between individual
scans were excluded (so there are gaps between scans).  These data
were used by the Naïve, Destriper, and HiRes (and SUPREME?).
\item{Set-2:} The TOD were not corrected for the detector array
  temperature drift; the “turn-around” data were included so there are
  no gaps between scans. These data were used by Scanamorphos,
  SANEPIC, and Unimap.
\end{description}

In order to facilitate the comparisons, we requested that all
map-makers project their maps in the same way. In particular, the
crota2 parameter should be 0 (north-up); the pixel sizes should be
those of the SPIRE standard (pixel = $6''$, $10''$, and $14''$
for PSW, PMW and
PLW maps); and the projection should be tangential in both the RA and
Dec directions (RA -- TAN, DEC -- TAN).

Because of the time constraint, not all map-makers processed all the
test cases (though some did). In Table~\ref{tbl:testcases}, 
the information on which
map-maker processed which test cases is provided with check marks.



==> chapter4_simulations.tex <==
\chapter{Simulations}\label{ch:simu}
Simulated data sets were generated for the SPIRE map-making tests. 
Compared with real data, a simulated data set has the advantage of 
possessing the ``truth'', namely the sky model, based on which the
simulation is carried out. The truth map provides an unbiased standard against
which test maps made by different map-makers are to be compared.
Allowing for the effects of noise in a given map, deviations from the truth 
can be used as objective measures for the bias introduced by the 
map-making process.

Each data set (a set of SPIRE Level1 scans over a sky region) was 
generated using two layers of data:
\begin{description}
\item{1)} noise layer --- real SPIRE observations (public data) of a dark field;
this allows the simulation to include both instrumental noise and confusion noise;
\item{2)} truth layer --- a sky-model map based either on (1) a real MIPS 24$\mu m$
map (beam-size $\sim 6''$) or (2) a map of artificial sources.
\end{description}

Sky-model maps in the ``truth layer'' are fine sampled (pixel of
$1.25"$ -- $1.5"$), convolved with SPIRE beams (sampled by 1" pixels), and
scaled to desired brightness. For those taken from the real MIPS
24$\mu m$ maps, the scaling factors were set to make the original
noise in the MIPS observations negligible compared to that in the
noise layer.
   
The simulation procedure is as follows: 
\begin{description}
\item{1)} take Level-1 data of a real SPIRE observation of a dark field
(i.e. the noise layer); 
\item{2)} take a sky-model map (i.e. the truth layer) and replace its WCS 
by that of the noise layer; 
\item{3)} obtain the RA and Dec for every sampling point in the Level-1 timelines of the noise layer;
\item{4)} then, read the signal in the sky-model map at the RA and Dec of a 
given sampling point in the noise layer, and add this signal to the signal
of that sampling point in the corresponding Level-1 timeline of the noise layer;
\item{5)} do step 4) for all sampling points in the noise layer.
\end{description}

In order to have comprehensive assessments for map-makers, we
requested that the simulated data sets should cover the following
parameter space for the SPIRE scan-map observations: (1) mapping mode
(nominal/parallel, scan speed, sampling rate), (2) source brightness,
(3) map size, (4) depth, (5) complexity of the extended emission.
 These simulations include instrumental
noise, confusion noise, and noise due to glitches. However, they do not include 
effects due to saturation, pointing error, 
photon noise contributed by very bright
sources. Also, the Level-1 timelines provided by the simulations are already
de-glitched using the standard SPIRE pipeline, which may not be desirable for
some map-makers (e.g. Unimap).
In total, we generated 8 simulated data sets (Table~\ref{tbl:simulations}).

\bigskip
\begin{table}[h]\footnotesize
%\begin{table}[h]\scriptsize
   \caption{Simulated Data Sets\label{tbl:simulations}}
\begin{tabular}{llllll}
\hline \\
Case & Mode & Truth Layer & Noise Layer & Depth & Bands \\
\hline \\
 1 & Nominal & artificial sources & Lockman-North   &  7 repeats & PSW, PMW, PLW\\
 2 & Nominal & cirrus region  & Lockman-North       &  7 repeats & PSW, PMW, PLW\\
 4 & Nominal & M51 & Lockman-North                  &  7 repeats & PSW, PMW, PLW\\
 5 & Fast-Scan & artificial sources & Lockman-SWIRE &  2 repeats & PSW, PLW\\
 6 & Fast-Scan & Galactic center  & Lockman-SWIRE   &  2 repeats & PSW, PLW\\
 8 & Parallel & artificial sources &  ELAIS N1      &  5 repeats & PSW, PLW\\
 9 & Parallel & Galactic center  &  ELAIS N1        &  5 repeats & PSW, PLW\\
10 & Parallel & cirrus region &  ELAIS N1           &  5 repeats & PSW, PLW\\
\hline \\
\end{tabular}
\end{table}


